ZeroPrompt: Scaling Prompt-Based Pretraining to 1,000 Tasks Improves Zero-Shot Generalization

We propose a multitask pretraining approach ZeroPrompt for zero-shot generalization, focusing on task scaling and zero-shot prompting. While previous models are trained on only a few dozen tasks, we scale to 1,000 tasks for the first time using real-world data. This leads to a crucial discovery that task scaling can be an efficient alternative to model scaling; i.e., the model size has little impact on performance with an extremely large number of tasks. Our results show that task scaling can substantially improve training efficiency by 30 times in FLOPs. Moreover, we present a prompting method that incorporates a genetic algorithm to automatically search for the best prompt for unseen tasks, along with a few other improvements. Empirically, ZeroPrompt substantially improves both the efficiency and the performance of zero-shot learning across a variety of academic and production datasets.

==> EMNLP 2022/exp.tex <==
\section{Experiments} \label{sec:exp}
\begin{table*}[t]
	\small
    \centering
    \begin{tabular}{cccccccc}
    \toprule
%    \hline\hline
         task type & task & \textbf{CPM-2} & \textbf{Pangu-$\alpha$} & \textbf{T5} & \textbf{RoBERTa} & \textbf{\proposed} & \textbf{T5} \\ 
         ~ & ~ & Zero-Shot & Zero-Shot & Zero-Shot & Finetuning & Zero-Shot & Finetuning \\
         \midrule
\multirow{3}{*}{\textbf{SENTI}}  & \scriptsize online\_shopping\_10cats & 80.60 & 61.99 & 71.88 & $95.30_{(0.42)}$ & $\textcolor{blue}{95.90}_{(0.24)}$ & $96.94_{(0.26)}$ \\ 
                              ~ & \scriptsize nlpcc2014\_task2         & 68.53 & 56.22 & 60.06 & $72.09_{(0.80)}$ & $\textcolor{blue}{80.49}_{(0.80)}$ & $80.67_{(0.21)}$ \\
                              ~ & \scriptsize SMP2019\_ECISA           & 29.04 & \textbf{40.41} & 31.21 & $69.45_{(1.65)}$ & $38.46_{(0.33)}$ & $74.15_{(0.30)}$ \\ \midrule
\multirow{1}{*}{\textbf{NEWS}}   & \scriptsize CCFBDCI2020              & 49.57 & 38.09 & 27.48 & $90.73_{(0.58)}$ & $\textbf{80.50}_{(1.68)}$ & $96.53_{(0.41)}$ \\ \midrule
\multirow{1}{*}{\textbf{INTENT}} & \scriptsize catslu\_traindev         & 62.63 & 46.65 & 11.27 & $91.09_{(2.33)}$ & $\textbf{90.48}_{(0.78)}$ & $94.42_{(0.66)}$ \\ \midrule
\multirow{1}{*}{\textbf{NLI}}    & \scriptsize ocnli\_public            & 33.76 & 38.58 & 30.51 & $54.70_{(0.53)}$ & $\textbf{46.16}_{(1.87)}$ & $58.15_{(1.61)}$ \\ \midrule
\multirow{2}{*}{\textbf{STS}}    & \scriptsize CBLUE-CHIP-STS           & 44.15 & 56.40 & 44.94 & $80.28_{(1.08)}$ & $\textbf{77.90}_{(0.59)}$ & $82.45_{(2.07)}$ \\
                              ~ & \scriptsize sohu-sts-B-ss            & 33.50 & 54.94 & 43.46 & $89.71_{(0.68)}$ & $\textbf{79.85}_{(1.03)}$ & $89.85_{(0.86)}$ \\ \midrule
\multirow{1}{*}{\textbf{QAM}}    & \scriptsize nlpcc2016-dbqa           & 49.90 & 56.08 & 51.69 & $56.31_{(1.51)}$ & $\textcolor{blue}{62.61}_{(3.64)}$ & $76.76_{(1.95)}$ \\ \midrule
\multirow{1}{*}{\textbf{PARA}}   & \scriptsize PAWS-X                   & 48.08 & 53.06 & 48.08 & $53.51_{(0.53)}$ & $\textcolor{blue}{54.90}_{(0.37)}$ & $59.04_{(0.51)}$ \\ \midrule
\multirow{1}{*}{\textbf{MRC}}    & \scriptsize cmrc2018\_public         & 8.51  & 11.61 & 5.94  & -                & $\textbf{35.50}_{(0.73)}$ & $61.00_{(0.80)}$ \\ \midrule
\multirow{2}{*}{\textbf{NER}}    & \scriptsize msra\_ner                & 3.11  & 9.81* & 21.44 & -                & $\textbf{58.17}_{(4.40)}$ & $65.37_{(2.65)}$ \\
                              ~ & \scriptsize CMeEE                   & 1.18     & 9.44* & 6.77  & -                & $\textbf{24.84}_{(0.94)}$ & $29.34_{(2.84)}$ \\ \midrule
\multirow{1}{*}{\textbf{SUMM}}    & \scriptsize EDU\_SUMM                & 1.05  & 10.02 & 2.21  & -                & $\textbf{14.80}_{(3.15)}$ & $16.97_{(2.11)}$ \\ \midrule
\multirow{1}{*}{\textbf{KEYS}}   & \scriptsize COTE-MFW                 & 1.29  & 4.91  & 7.05  & -                & $\textbf{50.34}_{(9.01)}$ & $79.35_{(1.08)}$ \\ \midrule
\multirow{1}{*}{\textbf{WSC}}    & \scriptsize cluewsc2020\_public      & \textbf{57.74} & 44.93 & 44.08 & $71.99_{(3.32)}$ & $47.98_{(4.18)}$ & $72.81_{(2.19)}$ \\ \midrule
\multirow{1}{*}{\textbf{APP}}  & \scriptsize iflytek\_public          & 4.77  & 7.85  & 1.69  & $50.34_{(0.61)}$ & $\textbf{26.14}_{(1.02)}$ & $53.33_{(1.05)}$ \\ \midrule
\multirow{10}{*}{\textbf{Production}} 
                                 & \scriptsize Return Commitment             & 36.28 & 51.83 & 53.28 & $96.16_{(0.21)}$ & $\textbf{95.53}_{(0.24)}$ & $96.78_{(0.62)}$\\   
                              ~ & \scriptsize Heating Supply               & 44.89 & 31.61 & 44.57 & $97.48_{(0.30)}$ & $\textcolor{blue}{99.22}_{(0.35)}$ & $98.91_{(0.59)}$\\
                              ~ & \scriptsize Return Amount                & 53.26 & 46.09 & 55.90 & $90.71_{(0.33)}$ & $\textbf{89.48}_{(0.56)}$ & $90.86_{(0.47)}$\\
                              ~ & \scriptsize Registration Discount             & 55.09 & 50.34 & 56.25 & $88.68_{(0.40)}$ & $\textbf{88.48}_{(0.51)}$ & $89.88_{(0.65)}$\\
                              ~ & \scriptsize Operation Guidance                & 57.97 & 47.71 & 54.52 & $90.78_{(0.35)}$ & $\textbf{78.24}_{(1.41)}$ & $92.80_{(0.84)}$\\
                              ~ & \scriptsize Promise for Refunding         & 46.80 & 49.35 & 48.57 & $93.71_{(0.24)}$ & $\textcolor{blue}{94.28}_{(0.56)}$ & $91.40_{(1.13)}$\\
                              ~ & \scriptsize Households Heating Plant      & 63.37 & 69.66 & 48.71 & $96.59_{(0.47)}$ & $\textcolor{blue}{98.22}_{(0.52)}$ & $97.39_{(0.59)}$\\
                              ~ & \scriptsize Refunding Amount              & 48.48 & 52.58 & 49.67 & $83.78_{(0.52)}$ & $\textcolor{blue}{88.03}_{(0.83)}$ & $83.74_{(1.67)}$\\
                              ~ & \scriptsize Cost Abatement                & 43.18 & 48.13 & 51.51 & $80.30_{(0.92)}$ & $\textcolor{blue}{81.88}_{(0.22)}$ & $81.40_{(1.02)}$\\
                              ~ & \scriptsize WeChat Operation              & 45.45 & 51.37 & 47.79 & $82.28_{(0.59)}$ & $\textbf{78.25}_{(0.26)}$ & $83.53_{(1.59)}$\\ \midrule
\multicolumn{2}{c}{\textbf{AVG}}                                     & 39.71 & 40.73 & 37.80 & -                & $\textbf{68.76}_{(1.48)}$ & $77.55_{(1.14)}$ \\
\multicolumn{2}{c}{\textbf{AVG excl. GEN}}                           & 48.05 & 47.90 & 44.42 & $80.73_{(0.85)}$ & $\textbf{76.04}_{(1.02)}$ & $83.72_{(0.94)}$ \\
\bottomrule
    \end{tabular}
    \caption{Main results of \proposed (1.5B) and other zero-shot/finetuning baselines. The numbers in brackets are the standard deviations of results with 5 different random seeds.
    -: We do not finetune RoBERTa on generation tasks because it is an encoder-only model.
    *: Only part of the test set is sampled for evaluation due to the computation burden. \textcolor{blue}{Blue} numbers indicate the cases where \proposed scores better than finetuned RoBERTa and \textbf{bold} numbers indicate the cases where \proposed achieves the best zero-shot performance. }
    \label{tab:main_results}
\end{table*}
% \begin{table*}[t]
% 	\small
%     \centering
%     \begin{tabular}{cccccccc}
%     \toprule
% %    \hline\hline
%          task type & \textbf{CPM-2} & \textbf{Pangu-$\alpha$} & \textbf{T5} & \textbf{RoBERTa} & \textbf{\proposed} & \textbf{T5} \\ 
%          ~ & ~ & Zero-Shot & Zero-Shot & Zero-Shot & Finetuning & Zero-Shot & Finetuning \\
%          \midrule
% \multirow{3}{*}{\textbf{SENTI}}  & 80.60 & 61.99 & 71.88 & $95.30_{(0.42)}$ & $\textcolor{blue}{95.90}_{(0.24)}$ & $96.94_{(0.26)}$ \\ 
%                               ~ & 68.53 & 56.22 & 60.06 & $72.09_{(0.80)}$ & $\textcolor{blue}{80.49}_{(0.80)}$ & $80.67_{(0.21)}$ \\
%                               ~ & 29.04 & \textbf{40.41} & 31.21 & $69.45_{(1.65)}$ & $38.46_{(0.33)}$ & $74.15_{(0.30)}$ \\ \midrule
% \multirow{1}{*}{\textbf{NEWS}}   & 49.57 & 38.09 & 27.48 & $90.73_{(0.58)}$ & $\textbf{80.50}_{(1.68)}$ & $96.53_{(0.41)}$ \\ \midrule
% \multirow{1}{*}{\textbf{INTENT}} & 62.63 & 46.65 & 11.27 & $91.09_{(2.33)}$ & $\textbf{90.48}_{(0.78)}$ & $94.42_{(0.66)}$ \\ \midrule
% \multirow{1}{*}{\textbf{NLI}}    & 33.76 & 38.58 & 30.51 & $54.70_{(0.53)}$ & $\textbf{46.16}_{(1.87)}$ & $58.15_{(1.61)}$ \\ \midrule
% \multirow{2}{*}{\textbf{STS}}    & 44.15 & 56.40 & 44.94 & $80.28_{(1.08)}$ & $\textbf{77.90}_{(0.59)}$ & $82.45_{(2.07)}$ \\
%                               ~ & 33.50 & 54.94 & 43.46 & $89.71_{(0.68)}$ & $\textbf{79.85}_{(1.03)}$ & $89.85_{(0.86)}$ \\ \midrule
% \multirow{1}{*}{\textbf{QAM}}    & 49.90 & 56.08 & 51.69 & $56.31_{(1.51)}$ & $\textcolor{blue}{62.61}_{(3.64)}$ & $76.76_{(1.95)}$ \\ \midrule
% \multirow{1}{*}{\textbf{PARA}}   & 48.08 & 53.06 & 48.08 & $53.51_{(0.53)}$ & $\textcolor{blue}{54.90}_{(0.37)}$ & $59.04_{(0.51)}$ \\ \midrule
% \multirow{1}{*}{\textbf{MRC}}    & 8.51  & 11.61 & 5.94  & -                & $\textbf{35.50}_{(0.73)}$ & $61.00_{(0.80)}$ \\ \midrule
% \multirow{2}{*}{\textbf{NER}}    & 3.11  & 9.81* & 21.44 & -                & $\textbf{58.17}_{(4.40)}$ & $65.37_{(2.65)}$ \\
%                               ~ & 1.18     & 9.44* & 6.77  & -                & $\textbf{24.84}_{(0.94)}$ & $29.34_{(2.84)}$ \\ \midrule
% \multirow{1}{*}{\textbf{SUMM}}   & 1.05  & 10.02 & 2.21  & -                & $\textbf{14.80}_{(3.15)}$ & $16.97_{(2.11)}$ \\ \midrule
% \multirow{1}{*}{\textbf{KEYS}}   & 1.29  & 4.91  & 7.05  & -                & $\textbf{50.34}_{(9.01)}$ & $79.35_{(1.08)}$ \\ \midrule
% \multirow{1}{*}{\textbf{WSC}}    & \textbf{57.74} & 44.93 & 44.08 & $71.99_{(3.32)}$ & $47.98_{(4.18)}$ & $72.81_{(2.19)}$ \\ \midrule
% \multirow{1}{*}{\textbf{APP}}    & 4.77  & 7.85  & 1.69  & $50.34_{(0.61)}$ & $\textbf{26.14}_{(1.02)}$ & $53.33_{(1.05)}$ \\ \midrule
% \multirow{10}{*}{\textbf{Production}} & 45.48 & 49.87 & 51.08 & $90.05_{(0.59)}$ & $\textbf{78.25}_{(0.26)}$ & $83.53_{(1.59)}$\\ \midrule
% \multicolumn{2}{c}{\textbf{AVG}}                                     & 39.71 & 40.73 & 37.80 & -                & $\textbf{68.76}_{(1.48)}$ & $77.55_{(1.14)}$ \\
% \multicolumn{2}{c}{\textbf{AVG excl. GEN}}                           & 48.05 & 47.90 & 44.42 & $80.73_{(0.85)}$ & $\textbf{76.04}_{(1.02)}$ & $83.72_{(0.94)}$ \\
% \bottomrule
%     \end{tabular}
%     \caption{Main results of \proposed and other zero-shot/finetuning baselines. The numbers in brackets are the standard deviations of results with 5 different random seeds.
%     -: We do not finetune RoBERTa on tagging and generation tasks.
%     *: Only part of the test set is sampled for evaluation due to the computation burden. \textcolor{blue}{Blue} numbers indicate the cases where \proposed scores better than finetuned RoBERTa and \textbf{bold} numbers indicate the cases where \proposed achieves the best zero-shot performance. }
%     \label{tab:main_results}
% \end{table*}


\subsection{Experiment Setups}

% \subsubsection{Models}
We compare \proposed with state-of-the-art large-scale Chinese pretrained models, Pangu-$\alpha$ (13B decoder)~\cite{zeng2021pangualpha}, CPM-2 (11B encoder-decoder)~\cite{Zhang2021cpm2}, and the finetuned RoBERTa-large model~\cite{liu2019roberta}. All finetuned baselines were trained one task at a time. We use a encoder-decoder model and apply both unsupervised pretraining and multitask prompted supervised pretraining. Training details of \proposed can be found in Appendix~\ref{appendix:training_detail}. 


% We repeat experiments, including multitask pretraining and finetuning of RoBERTa, T5, five times with different random seeds to reduce variance.
% Training and test datasets details are presented in Sec~\ref{subsection:Datasets}.
% Details regarding evaluation metrics can be seen in Appendix~\ref{subsec:appendix_metric}.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.40\textwidth]{figures/task_scale_cross_domain.pdf}
%     \includegraphics[width=0.40\textwidth]{figures/task_scale_cross_type.pdf}
%     \caption{Out-of-domain (left) and cross-task-type (right) zero-shot performance with different number of training tasks. Few-shot validation is \textbf{not} employed to exclude potential confounding factors from the study.}
%     \label{fig:task_scale_cross_domain_task_type}
% \end{figure*}

\subsection{Main Results}
\subsubsection{Power of Task Scaling} 
% \zy{Should this be put into Experiments? This should be the main results I guess.}
\label{subs: scale_experiment}

% We explore the limits of zero-shot performance of multitask prompted pretraining, using over 1,000 tasks from 10 domains. 
% Since model scaling has been shown to have significant impact on zero-shot performance~\cite{NEURIPS2020_gpt3}, we also provide the results of three models with 0.4B, 1.5B and 12B parameters.
To study the law of task scaling, we trained \proposed on a mixture of public data and production data, and increased the number of production training tasks from 20 to 800.
Zero-shot performance on unseen production test tasks are presented in Figure~\ref{fig:main_cmp}.
Larger models have much better zero-shot performance with a limited number of training tasks.
However, the performance gains from larger models decrease when more training tasks are added. 
% The 0.4B model achieves a score of 87 with 800 training tasks, which scores better than the 12B model with only 200 training tasks. 
Generally, if we scale the number of training tasks, small models can still achieve impressive zero-shot performance, substantially improving training efficiency by 30 times in FLOPs (0.4B vs 12B) as well as the serving efficiency.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.40\textwidth]{figures/task_scale_cross_type.pdf}
    \caption{Zero-shot performance on cross-task-type tasks with different number of training tasks. }
    \label{fig:task_scale_cross_task_type}
\end{figure}

\subsubsection{Comparison with Other Baselines}

% In this section, we compare \proposed with other strong zero-shot and fully-supervised baselines on unseen testing datasets.
% Note that due to limited space, only part of the reserved testing tasks, specifically 17 academic and 10 production datasets, are included in Table~\ref{tab:main_results} for comparison.

Results on the reserved testing tasks are shown in Table~\ref{tab:main_results}, in the zero-shot setting, \proposed significantly improves the performance of T5 from 37.80 to 68.76 with a boost of 30.96 points, outperforming previous PTMs, CPM-2 and Pangu-$\alpha$, by a large margin of 28 points.
Notably, \proposed is comparable to or even better than a finetuned RoBERTa-large model on some academic and production datasets.
Compared to the overall score of the finetuned RoBERTa, \proposed is only 4.7 points short. This is quite ecstatic considering that \proposed did not use any labeled data for tuning. 
% The finetuned T5 is better than RoBERTa, and the gap between \proposed and the finetuned T5 is less than 8 points.

\subsection{Discussions}
\subsubsection{Task Scaling vs Sample Scaling}

While task scaling by definition also increases the number of training samples, we also decouple the effects of task scaling and sample scaling in Table \ref{tab:task_num_data_num}. The numbers of total samples are the same for ``80 tasks with 1280 shots'' and ``800 tasks with 128 shots'', but the latter shows considerably better performance---4.8 and 3.0 points improvement for the 0.4B model and the 1.5B model, respectively.
% Moreover, task scaling closes the gap between different model sizes; this effect is less prominent for sample scaling.

% We also study the efficiency of task scaling and sample scaling, and the results are given in Table~\ref{tab:task_num_data_num}. Although the number of data points for 100 tasks with 1280-shot is the same as 800 tasks with 128-shot, the latter shows considerable better performance by 4.8, 3.0 and - points for models with 0.4B, 1.5B and 12B parameters, respectively. The empirical results show that task scaling is more efficient than sample scaling to boost the zero-shot performance, especially for small and medium-sized models.

\subsubsection{Unsupervised Data vs Supervised Data}
\begin{table}[t]
\footnotesize
    \centering
    \begin{tabular}{cccc}
    \toprule
    Model size & \makecell[c]{100 tasks \\ 128-shot} & \makecell[c]{80 tasks \\ 1280-shot} & \makecell[c]{800 tasks \\ 128-shot} \\
    \midrule
    0.4B & 70.5 & 82.5 & 87.3 \\
    1.5B & 84.0 & 86.2 & 89.2 \\
    12B  & 84.8 & 88.7 & 89.4 \\
    \bottomrule
    \end{tabular}
    \caption{Task scaling vs sample scaling.}
    \label{tab:task_num_data_num}
\end{table}


\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{cccc}
\toprule
    Model & 0.4B & 1.5B & 12B \\ \midrule
    LM loss & 1.9 & 1.7 & 1.5 \\
    Sup loss & 0.19 & 0.17 & 0.19 \\
\bottomrule
\end{tabular}
\caption{Language modeling (LM) and supervised (Sup) validation loss of models with different sizes.}
\label{tab:loss}
\end{table}

Zero-shot performance is attributed to both supervised tasks and the LM task. As we increase the number of supervised tasks, they outweigh the LM task. Meanwhile, these supervised tasks have much less data to fit than the LM task, which makes smaller models viable choices.
Table \ref{tab:loss} shows that smaller models have similar losses on supervised tasks but higher losses on LM, compared to larger models. This explains why task scaling can be an alternative to model scaling. 


\subsubsection{Effect of Task Distribution}
To validate the zero-shot performance on cross-task-type tasks, we select production tasks from two task types for testing and the rest for training, as presented in Figure~\ref{fig:task_scale_cross_task_type}. It can be seen that task scaling still leads to significant improvement of zero-shot performance on cross-task-type tasks. On the other hand, Figure~\ref{fig:task_scale_general_test_1b} shows the zero-shot performance on public datasets. For some tasks like INTENT, the scaling of production tasks is helpful, but the result could be different for other tasks like SENTI. The average performance of all public datasets does not increase monotonically with more training tasks. We suppose the reason is that the task distribution of production data is different from that of public tasks. Therefore, only part of public tasks benefit from the scaling of production training tasks. We also study the effect of cross task type transfer on public tasks, the results can be found in Appendix~\ref{appendix:cross_type_transfer}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.40\textwidth]{figures/task_scale_general_test_1b.pdf}
    \caption{Zero-shot performance of 1.5B model on public datasets with different number of production training tasks.}
    \label{fig:task_scale_general_test_1b}
\end{figure}

\section{Conclusions}
In this paper, we propose \proposed, a multitask prompted pretraining method that significantly improves the zero-shot generalization ability of language models. In our experiments, we collect over 1,000 real-world production tasks to study the task scaling law. We find that on our considered datasets, the zero-shot performance gap between small and large models becomes less significant when having more training tasks. As a result, task scaling can substantially improve training and serving efficiency.

\section{Limitations}
% We show that task scaling, which could now be seen as an alternative to model scaling, improves both the efficiency and performance of zero-shot learning. 
Our results regarding the effect of task scaling on zero-shot performance still have a few limitations.
% and it is possible that zero-shot performance could be further improved by studying those problems in the future.
Specifically, We control our study by only increasing the number of tasks collected from our production system, and they might only represent a subset of all the NLP problems. In addition, for different testing tasks in the public datasets, the zero-shot performance might not increase with the scaling of production training tasks. Therefore, the conclusion that task scaling can significantly boost zero-shot performance is limited to the case where training and test tasks share some similarity in distribution, but not a general conclusion for arbitrary distributions.
It also remains an open problem as how to quantitatively characterize the distribution similarity between training and test tasks.
% stands on our collected production tasks, but not a general conclusion.
% The problem of how to choose a better training task distribution is left for future work.
% , since it is not relevant to our main focus.
% 2) Our tasks are not exhaustive, because our real-world production data might only represent a subset of all the NLP problems.
% However, it is challenging to collect more diverse data for the study of task scaling, because publicly available data is often limited in terms of the number of tasks. Therefore, we choose to use production data to initiate such a study.
% 3) The conclusion that task scaling can significantly boost zero-shot performance stands on our collected production datasets, but not a general conclusion for all NLP tasks.
We hope our results could encourage future work on addressing these limitations to further explore the potential of zero-shot learning.
% We will also publish related data to facilitate research in this direction.





% Entries for the entire Anthology, followed by custom entries
\bibliography{custom}
\bibliographystyle{acl_natbib}


==> EMNLP 2022/intro.tex <==
\section{Introduction}

% Pretrained language models, such as BERT \cite{devlin-etal-2019-bert}, XLNet \cite{yang2019xlnet}, T5 \cite{JMLR:v21:20-074}, and GPT \cite{radf2019lmmultitask}, are often finetuned for downstream natural language processing tasks, which has been shown to improve performance over non-pretrained models. However, this pretraining-finetuning paradigm still relies on a relatively large set of labeled data for each downstream task to obtain competitive performance. 

% Generalizing language models to a variety of downstream tasks draws large amount of attention. 
Recent progress like GPT-3 \cite{NEURIPS2020_gpt3} demonstrates the possibility of prompting on larger-scale models for zero-shot learning, but the performance of zero-shot generalization still falls short on many tasks compared to fully-supervised finetuning.
Further, other works proposed to include a set of supervised tasks into pretraining~\cite{zhong2021adapting,wei2021finetuned,sanh2021multitask}, and prompts are often used in the framework to unify the tasks.
\citet{zhong2021adapting} converted different datasets into a unified ``yes/no'' question answering format with label descriptions. FLAN~\cite{wei2021finetuned} extended the scope by considering more task types and a larger model. T0~\cite{sanh2021multitask} collected a large set of diverse prompts for each task to further enhance performance.

% wang2022benchmarking

Despite the effects of model scaling and prompts scaling~\cite{wei2021finetuned,sanh2021multitask} have been explored, only dozens of training tasks are exploited in these works. It is still not clear how scaling the number of training tasks to hundreds even thousands of tasks affects the performance of multitask pretraining. We hypothesize that task scaling plays an important role in training generalizable zero-shot systems and explore the limits of task scaling using 1,000 tasks. Interestingly, our empirical study reveals that task scaling can be an efficient alternative to model scaling, as shown in Figure \ref{fig:main_cmp}.
With an extremely large number of training tasks, the model size has less impact on performance.
A 0.4B model can achieve comparable zero-shot performance to that of a 12B model, improving training efficiency by 30 times in terms of FLOPs and the serving efficiency as well. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/intro_figure.pdf}
    \caption{Task scaling vs model scaling. The horizontal axis is the number of training tasks, and the vertical axis is the zero-shot performance on unseen tasks.
    % Task scaling is an efficient alternative to model scaling.
    % With an extremely large number of training tasks, the model size has less impact on performance.
    % Moreover, task scaling consistently improves performance at various model scales.
    RoBERTa-Large was finetuned in a fully-supervised manner, while Pangu Alpha, CPM-2 and our ZeroPrompt were zero-shot prompted.
    % We report zero-shot performance without any labeled data.
}
    \label{fig:main_cmp}
\end{figure}

Our contributions can be summarized as follows. 
\begin{itemize}
    \item We scale the number of tasks to 1,000 in multitask pretraining for the first time. Our study reveals a crucial finding that on the datasets we consider, task scaling is an efficient alternative to model scaling.
    \item Our experiments demonstrate that task scaling improves both the efficiency and the performance of zero-shot learning.
\end{itemize}

==> EMNLP 2022/method.tex <==
\section{\proposed}
We follow the same framework of multitask zero-shot learning in ~\cite{wei2021finetuned,sanh2021multitask}, where models are pretrained on a variety of tasks and then tested on held-out unseen tasks. 


\begin{table}[!t]
\small
\centering
\begin{tabular}{lc}
\toprule
\textbf{Task type} & \textbf{\# of Tasks}  \\
\midrule
\scriptsize Sentiment Analysis (\textbf{SENTI})                 & 17 (4,13)          \\ 
\scriptsize News Classification (\textbf{NEWS})                 & 9  (4,5)          \\
\scriptsize Intent Classification  (\textbf{INTENT})            & 4  (1,3)      \\
\scriptsize Natural Language Inference. (\textbf{NLI})          & 2  (1,1)   \\ 
\scriptsize Sentence Similarity.  (\textbf{STS})                & 13 (3,10)  \\ 
\scriptsize Paraphrase (\textbf{PARA})                          & 1  (0,1)     \\ 
\scriptsize Question Answer Matching.  (\textbf{QAM})           & 1  (0,1)   \\
\scriptsize Machine Reading Comprehension (\textbf{MRC})        & 10 (5,5)    \\ 
\scriptsize Name Entity Recognition   (\textbf{NER})            & 9  (3,6)\\
\scriptsize Summarization  (\textbf{SUMM})                       & 9  (3,6)\\
\scriptsize Keywords       (\textbf{KEYS})                      & 3  (0,3) \\ 
\scriptsize Winograd Schema Challenge  (\textbf{WSC})           & 1  (0,1) \\ 
\scriptsize App Classification    (\textbf{APP})                & 1  (0,1) \\ 
\scriptsize Production tasks (\textbf{Objection})                                    & 110 (85,25) \\
\scriptsize Production tasks (\textbf{Profile})                                     & 345 (268,77) \\
\scriptsize Production tasks (\textbf{Execution})                                     & 310 (240,70) \\
\scriptsize Production tasks (\textbf{Mention})                                     & 125 (97,28) \\
\scriptsize Production tasks (\textbf{Violation})                                     & 90 (70,20) \\
\scriptsize Production tasks (\textbf{Acception})                                     & 50 (38,12) \\
\midrule
In total                                            &  1110 (824,286) \\
\bottomrule
\end{tabular}
\caption{The number of tasks for each task type. Numbers in brackets stand for the number of tasks for training and testing, respectively. e.g. SENTI has 4 tasks for training and 13 for testing.}
\label{tab:datasets_used_count}
\end{table}


% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/paradigm.pdf}
%     \caption{Different NLP paradigms. (a) Traditional pretraining-finetuning paradigm, requiring considerable labeled data for finetuning (b) \proposed pipeline, only need a tiny validation set for prompt search.}
%     \label{fig:compare_figure}
% \end{figure*}


% \subsubsection{Datasets}
\subsection{Datasets for Scaling to 1,000+ Tasks}\label{subsection:Datasets}
We collected 80 public Chinese NLP tasks and further
% the Chinese Language Understanding Evaluation benchmark (CLUE),
% the Chinese Natural Language Processing Conference Competition (NLPCC),
% and many other well-known Chinese NLP competitions.
% Considering that the number of open-source datasets is still insufficient for studying task scaling,
acquired over 1,000 real-world datasets from our production systems to investigate the task number scaling law. The number of tasks in each task type is listed in Table~\ref{tab:datasets_used_count}, where we define task types following previous work and intuitive knowledge.
The task taxonomy of the production datasets is presented in Appendix~\ref{appendix:datasets}, consisting of 6 task types from 10 different domains.


We split the public datasets and the production datasets into training tasks and testing tasks, as shown in Table~\ref{tab:datasets_used_count}.
Different from FLAN~\cite{sanh2021multitask} or T0~\cite{wei2021finetuned}, our test set contains a more diverse set of task clusters.
% , and the number of test datasets is twice that of train sets for proper evaluation.
% We argue that this is the practical real-world setting with a large number of different unseen tasks in the test set.
Detailed train/test splits can be found in Table~\ref{tab:summary_datasets}.
To simulate real-world NLP production systems at scale, where the costs for data labeling are expensive, we sample 128 examples per class for each classification task and 256 examples for each generation task to build the training set\footnote{Only 512 data points are sampled for the iflytek dataset as it has over 100 classes}.


\subsection{Prompt Design}
Although large-scale pretrained models with prompting show promising results on zero-shot generalization to unseen tasks without any labeled data, prompt design is of vital importance to their performance. We applies both the hard prompt, which is composed of label candidates and task descriptions, and the soft prompt at the mulitask pretraining stage, details of prompt design can be found in Appendix~\ref{appendix:prompt_design}.


==> EMNLP 2022/related.tex <==
\section{Related Work}


% \subsection{Prompting}
% Recently, prompt-based learning has been widely explored as it can perform few-shot or even zero-shot learning on many tasks~\cite{schick-schutze-2021-exploiting,gao-etal-2021-making,le-scao-rush-2021-many}.
% Prompt-based learning bridges the gap between pretraining and finetuning objectives by stitching the text input $X$ with a prompt template and augmenting the label output $y$ as a text string, such that the input and the output can be constructed in a sentence completion task form.
% Previous methods can be categorized into two types, discrete prompting~\cite{shin-etal-2020-autoprompt,gao-etal-2021-making,mishra2021reframing} and continuous prompting~\cite{liu2021gpt,han2021ptr}:
% The former requires users to provide handcrafted templates~\cite{shin-etal-2020-autoprompt,le-scao-rush-2021-many}, while the latter inserts learnable parameters in the template and directly optimize them during training \cite{han2021ptr,liu2021gpt,lester2021power}.

% In the zero-shot learning setting, discrete prompting requires human efforts to provide manual prompts. 
% Additionally, the settings from previous work where no validation set is used to evaluate task performance are not practical to production NLP systems which require robustness. 
% Continuous prompting requires updating the learnable parameters using labeled data for the tuning phase and thus suffers from requiring even more human efforts in labeling. 
% Instead, our prompting method targets better zero-shot generalization automatically with a few labeled samples per task only used for validation.

% \subsection{Pretraining and Zero-shot Generalization}
Pretrained language models, like BERT~\cite{devlin-etal-2019-bert}, XLNet~\cite{yang2019xlnet}, T5~\cite{JMLR:v21:20-074} and GPTs~\cite{NEURIPS2020_gpt3,radf2019lmmultitask}, have achieved strong performance on various NLP tasks. In some cases, pretrained models can perform well with only a few training samples~\cite{liu2021gpt,schick-schutze-2021-exploiting}, or even without any training sample~\cite{Shen2021ConterfactualGZ,sanh2021multitask}. 
% These works mainly focus on unsupervised pretraining on a large-scale corpus.


It has been shown that augmenting unsupervised pretraining with supervised data can significantly improve task performance during finetuning~\cite{chen2020big, gururangan2020don}.
Some recent studies followed this idea and obtained improved few-shot or zero-shot generalization in the same manner.
For instance, Mishra et al.~\cite{swaroopmishra2021crosstask} built a dataset with task instructions, and
CROSSFIT~\cite{ye2021crossfit} introduced a repository of few-shot text-to-text tasks.
FLAN~\cite{wei2021finetuned} and T0~\cite{sanh2021multitask} applied instruction-tuning of many tasks with 137B and 11B parameters, respectively. 
ExT5~\cite{2021ext5} applies multitask pretraining as well, but it focuses on multitask cotraining transfer instead of zero-shot generalization.
% to a large-scale decoder model with 137B parameters, while T0~\cite{sanh2021multitask} trained an encoder-decoder model with 11B parameters on a large number of professionally crowd-sourced prompts.
Our \proposed utilizes labeled data in the pretraining phase, and we aim at studying the task scaling law of zero-shot generalization by adopting 1,000 real-world tasks.


% \subsection{Domain Generalization}
% Domain generalization addresses the model's ability to generalize to unseen test domains with data from several different but related domains~\cite{Wang2021GeneralizingTU}.
% Previous approaches in domain generalization are mainly based on gradient operations~\cite{gulrajani2020search,arjovsky2019invariant,mansilla2021domain,kim2021selfreg} or disentanglement learning~\cite{wang2020cross,peng2020domain2vec,peng2019domain}. 
% Different from the above problem formulation, we focus on zero-shot task generalization to unseen tasks with the benefit of prompting to unify different NLP tasks by having the same data format.
